Search for the Decay of the Higgs Boson to Charm Quarks with the ATLAS Experiment

A direct search for the Standard Model Higgs boson decaying to a pair of charm quarks is presented. Associated production of the Higgs and $Z$ bosons, in the decay mode $ZH\rightarrow \ell^+ \ell^- c \bar{c}$ is studied. A dataset with an integrated luminosity of 36.1 fb$^{-1}$ of $pp$ collisions at $\sqrt{s}=13$ TeV recorded by the ATLAS experiment at the LHC is used. The $H\rightarrow c\bar{c}$ signature is identified using charm-tagging algorithms. The observed (expected) upper limit on $\sigma(pp \rightarrow ZH) \times \mathcal{B}(H \rightarrow c\bar{c})$ is 2.7 ($3.9^{+2.1}_{-1.1}$) pb at the 95% confidence level for a Higgs boson mass of 125 GeV, while the Standard Model value is 26 fb.

==> Acknowledgements.tex <==
% Acknowledgements for papers with collision data
% Version 14-Feb-2018

% Standard acknowledgements start here
%----------------------------------------------
We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC, Australia; BMWFW and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP, Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC, China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic; DNRF and DNSRC, Denmark; IN2P3-CNRS, CEA-DRF/IRFU, France; SRNSFG, Georgia; BMBF, HGF, and MPG, Germany; GSRT, Greece; RGC, Hong Kong SAR, China; ISF, I-CORE and Benoziyo Center, Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; NWO, Netherlands; RCN, Norway; MNiSW and NCN, Poland; FCT, Portugal; MNE/IFA, Romania; MES of Russia and NRC KI, Russian Federation; JINR; MESTD, Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa; MINECO, Spain; SRC and Wallenberg Foundation, Sweden; SERI, SNSF and Cantons of Bern and Geneva, Switzerland; MOST, Taiwan; TAEK, Turkey; STFC, United Kingdom; DOE and NSF, United States of America. In addition, individual groups and members have received support from BCKDF, the Canada Council, CANARIE, CRC, Compute Canada, FQRNT, and the Ontario Innovation Trust, Canada; EPLANET, ERC, ERDF, FP7, Horizon 2020 and Marie Sk{\l}odowska-Curie Actions, European Union; Investissements d'Avenir Labex and Idex, ANR, R{\'e}gion Auvergne and Fondation Partager le Savoir, France; DFG and AvH Foundation, Germany; Herakleitos, Thales and Aristeia programmes co-financed by EU-ESF and the Greek NSRF; BSF, GIF and Minerva, Israel; BRF, Norway; CERCA Programme Generalitat de Catalunya, Generalitat Valenciana, Spain; the Royal Society and Leverhulme Trust, United Kingdom.

The crucial computing support from all WLCG partners is acknowledged gratefully, in particular from CERN, the ATLAS Tier-1 facilities at TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France), KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain), ASGC (Taiwan), RAL (UK) and BNL (USA), the Tier-2 facilities worldwide and large non-WLCG resource providers. Major contributors of computing resources are listed in Ref.~\cite{ATL-GEN-PUB-2016-002}.
%----------------------------------------------



==> ZHccPaper-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

% Title
\AtlasTitle{Search for the Decay of the Higgs Boson to Charm Quarks with the ATLAS Experiment}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page,
% and line numbers.
% Comment or remove in final version.
\AtlasVersion{2.5}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
A direct search for the Standard Model Higgs boson decaying to a pair of charm quarks is presented. Associated production of the Higgs and $Z$ bosons, in the decay mode $ZH\rightarrow \ell^+ \ell^- c \bar{c}$ is studied. A dataset with an integrated luminosity of 36.1 \ifb\ of $pp$ collisions at $\rts=13\,\TeV$ recorded by the ATLAS experiment at the LHC is used. The $H\rightarrow c\bar{c}$ signature is identified using charm-tagging algorithms. The observed (expected) upper limit on $\sigma(pp \rightarrow ZH) \times \mathcal{B}(H \rightarrow c\bar{c})$ is 2.7 ($3.9^{+2.1}_{-1.1}$)~pb at the 95\% confidence level for a Higgs boson mass of 125~GeV, while the Standard Model value is 26~fb.
%abstract can be max 600 chars, be careful~
%The analysis procedure is validated by a measurement of the yield of $WZ$ and $ZZ$ production with $Z\rightarrow c \bar{c}$ and $W\to cs$ in the same final states as the Higgs boson search, from which the ratio of the observed signal yield to the Standard Model expectation is found to be $XX \pm YY \mathrm{(stat.)} \pm ZZ \mathrm{(syst.)}$.
}

% Author - this does not work with revtex (add it after \begin{document})
\author{The ATLAS Collaboration}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{HIGG-2017-01}

% CERN preprint number
% \PreprintIdNumber{CERN-PH-2016-XX}

% ATLAS date - arXiv submission; usually filled in by the Physics Office
% \AtlasDate{\today}

% ATLAS heading - heading at top of title page. Set for TDR etc.
% \AtlasHeading{ATLAS ABC TDR}

% arXiv identifier
% \arXivId{14XX.YYYY}

% HepData record
% \HepDataRecord{ZZZZZZZZ}

% Submission journal and final reference
\AtlasJournalRef{Phys. Rev. Lett. 120 (2018) 211802}
\AtlasDOI{DOI:10.1103/PhysRevLett.120.211802}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% List of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
\AtlasCoverSupportingNote{Search for $H\rightarrow c\bar{c}$ decays in associated $ZH$ production}{http://cds.cern.ch/record/2237398}
% \AtlasCoverSupportingNote{Short title note 2}{https://cds.cern.ch/record/YYYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
\AtlasCoverCommentsDeadline{20 December 2017}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
\AtlasCoverAnalysisTeam{Adrian Buzatu, Tingting Cao, Andrew Chisholm, Yara Coutinho, Erez Etzion, Tobias Golling, Heather Gray, Eilam Gross, Marie Lanfermann, Kostas Nikolopoulos, Elliot Reynolds, Joe Taenzer, Guy Koren, Elisabeth Schopf, Jonathan Shlomi}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
% Give either all members at once (then they appear on one line), or separately
% \AtlasCoverEdBoardMember{EdBoard~Chair~(chair), EB~Member~1, EB~Member~2, EB~Member~3}
\AtlasCoverEdBoardMember{Wouter Verkerke~(chair)}
\AtlasCoverEdBoardMember{Jean-François Grivaz}
\AtlasCoverEdBoardMember{Matthias Danninger}
% \AtlasCoverEdBoardMember{EB~Member~3}

% A PUB note has readers and not an EdBoard -- give their names here (one line or several entries)
% \AtlasCoverReaderMember{Reader~1, Reader~2}
% \AtlasCoverReaderMember{Reader~1}
% \AtlasCoverEdBoardMember{Reader~2}

% Editors egroup
\AtlasCoverEgroupEditors{atlas-higg-2017-01-editors@cern.ch}

% EdBoard egroup
\AtlasCoverEgroupEdBoard{atlas-higg-2017-01-editorial-board@cern.ch}

